Fermionic T-duality and U-duality in type II supergravity

This thesis deals with the two duality symmetries of N=2 D=10 supergravity theories that are descendant from the full superstring theory: fermionic T-duality and U-duality. The fermionic T-duality transformation is applied to the D-brane and pp-wave solutions of type IIB supergravity. New supersymmetric solutions of complexified supergravity are generated. We show that the pp-wave yields a purely imaginary background after two dualities, undergoes a geometric transformation after four dualities, and is self-dual after eight dualities. Next we apply six bosonic and six fermionic T-dualities to the AdS_4 x CP^3 background of type IIA supergravity, which is relevant to the current research in the amplitude physics. This helps to elucidate the potential obstacles in establishing the self-duality, and quite independently from that shows us that fermionic T-dualities may be degenerate under some circumstances. Finally, we make a step towards constructing a manifestly U-duality covariant action for D=10 supergravities by deriving the generalized metric for a D1-brane. This is a single structure that treats brane wrapping coordinates on the same footing as spacetime coordinates. It turns out that the generalized metric of a D-string results from that of the fundamental string if one replaces the spacetime metric with the open string metric. We also find an antisymmetric contribution to the generalized metric that can be interpreted as a noncommutativity parameter.

==> titlepage.tex <==
\vspace{1truecm}

\begin{center}{\LARGE \bf Fermionic T-duality}\end{center}

\vspace{1truecm}
\thispagestyle{empty} 
\centerline{{\large \bf Ilya Bakhmatov ${}^{\dag}$}}

\vspace{.4cm}
\centerline{{\it A thesis submitted for the degree of Doctor of Philosophy}}
\vspace{2cm}

\centerline{{\it ${}^\dag$ Centre for Research in String Theory, School of Physics}}
\centerline{{\it Queen Mary University of London}} 
\centerline{{\it Mile End Road, London E1 4NS, UK}}
\centerline{{i.bakhmatov@qmul.ac.uk}}

\vspace{.4cm}
